A Simple Framework for Open-Vocabulary Segmentation and Detection

We present OpenSeeD, a simple Open-vocabulary Segmentation and Detection framework that jointly learns from different segmentation and detection datasets. To bridge the gap of vocabulary and annotation granularity, we first introduce a pre-trained text encoder to encode all the visual concepts in two tasks and learn a common semantic space for them. This gives us reasonably good results compared with the counterparts trained on segmentation task only. To further reconcile them, we locate two discrepancies: $i$) task discrepancy -- segmentation requires extracting masks for both foreground objects and background stuff, while detection merely cares about the former; $ii$) data discrepancy -- box and mask annotations are with different spatial granularity, and thus not directly interchangeable. To address these issues, we propose a decoupled decoding to reduce the interference between foreground/background and a conditioned mask decoding to assist in generating masks for given boxes. To this end, we develop a simple encoder-decoder model encompassing all three techniques and train it jointly on COCO and Objects365. After pre-training, our model exhibits competitive or stronger zero-shot transferability for both segmentation and detection. Specifically, OpenSeeD beats the state-of-the-art method for open-vocabulary instance and panoptic segmentation across 5 datasets, and outperforms previous work for open-vocabulary detection on LVIS and ODinW under similar settings. When transferred to specific tasks, our model achieves new SoTA for panoptic segmentation on COCO and ADE20K, and instance segmentation on ADE20K and Cityscapes. Finally, we note that OpenSeeD is the first to explore the potential of joint training on segmentation and detection, and hope it can be received as a strong baseline for developing a single model for both tasks in open world.

==> iccv2023AuthorKit/resources/imgs/intro_fig.tex <==
\begin{figure*}[h!]
    \centering
    % \vspace{4pt}
    \includegraphics[width=\linewidth]{iccv2023AuthorKit/resources/imgs/introfig_v2.pdf}
    \caption{Some visualization of our segmentation results.}%\Jianwei{source image is too small?}
    \label{fig:decoded_mask}
    % \vspace{-0.8cm}
\end{figure*}

==> iccv2023AuthorKit/resources/imgs/match_compare.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{iccv2023AuthorKit/resources/imgs/cond_matching.pdf}
    % \vspace{-0.2cm}
    \caption{A comparison of }
    \label{fig:cond matching}
    % \vspace{-0.8cm}
\end{figure}

==> iccv2023AuthorKit/resources/imgs/sota_fig.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]
    {iccv2023AuthorKit/resources/imgs/sota.pdf}
    % {iccv2023AuthorKit/resources/imgs/attention_mask.pdf}
    % \vspace{-0.2cm}
    \caption{Our \ourmodel{} model outperforms previous state-of-the-art methods (listed below each gray bar) on eight benchmarks in zero-shot and task-specific transfer settings.}
    \label{fig:teaser}
    \vspace{-3pt}
\end{figure}

==> iccv2023AuthorKit/resources/tabels/ablation_teacher_matching.tex <==
% \usepackage[normalem]{ulem}
% \usepackage{multirow}
% \usepackage{colortbl}
% \usepackage{booktabs}
% \usepackage{hhline}


\begin{table}
\centering
\tablestyle{3pt}{0.95}
\setlength{\extrarowheight}{0pt}
\addtolength{\extrarowheight}{\aboverulesep}
\addtolength{\extrarowheight}{\belowrulesep}
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\caption{\textbf{Ablation} of the effectiveness of conditioned mask matching. We conduct experiment with or without conditioned mask matching on two commonly used open-vocabulary segmentation datasets ADE20K and Cityscapes. "w/o" is short for without.}
\label{tab:task_transfer}
\begin{adjustbox}{width=0.45\textwidth,center}

\begin{tabular}{l|cclc|cclc|} 
\toprule
\multirow{2}{*}{Method}                        
&\multicolumn{4}{c|}{ADE}   & \multicolumn{4}{c}{COCO} \\
& PQ  & mask AP  & box AP & {mIoU}   & PQ & mask AP&box AP & mIoU \\ 
\hline

\ourmodel{}-SwinT w/o condition  &  19.4 & 13.6 &16.7&22.9&55.0&52.3&47.5& 63.9                                           \\
\ourmodel{}-SwinT-condition &  19.6 & 14.2&17.2&23.1&55.2& 51.9 &47.3& 63.7                                           \\

\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:ablation:online matching}
\end{table}

==> iccv2023AuthorKit/resources/tabels/metrics_ov.tex <==
% \usepackage[normalem]{ulem}
% \usepackage{multirow}
% \usepackage{colortbl}
% \usepackage{booktabs}
% \usepackage{hhline}


\begin{table*}
\centering
\tablestyle{3pt}{0.95}
\setlength{\extrarowheight}{0pt}
\addtolength{\extrarowheight}{\aboverulesep}
\addtolength{\extrarowheight}{\belowrulesep}
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\caption{open vocabulary metrics}
\label{tab:task_transfer}
\begin{tabular}{l|cclc|cclc|} 
\toprule
\multirow{2}{*}{Method}                        
&\multicolumn{4}{c|}{ADE}   & \multicolumn{4}{c|}{ADE} \\
& PQ  & mask AP  & box AP & {mIoU}    & PQ-ov & mask AP-ov & box AP-ov & mIoU-ov \\ 
\cline{1-9}

X-Decoder  &  18.8  &9.8 &-&25.0&&&                                             \\
\ourmodel  &  39.7 & 26.4 &&&&&&                                             \\
\ourmodel-flip1  &  39.7 & 26.4 &&&&&&                                             \\
\ourmodel-flip2  &  39.7 & 26.4 &&&&&&                                             \\

\bottomrule
\end{tabular}
\end{table*}

==> iccv2023AuthorKit/resources/tabels/task_transfrer2.tex <==
% \usepackage[normalem]{ulem}
% \usepackage{multirow}
% \usepackage{colortbl}
% \usepackage{booktabs}
% \usepackage{hhline}

\begin{table*}
\caption{\textbf{Task-specific transfer} of \ourmodel{} to different segmentation and VL tasks. We directly evaluate the COCO performance without finetuning. Note: ``$-$" denotes the model has the capability for the task but does not have number reported. ``-" means the model does not have the ability for the specific task.  ``a$\lvert$b" means ``pretrain$\lvert$finetune". $\star$ means it is the test set results.  The results in the bracket are trained with 1280$\times$1280 image size.}
\label{tab:task_transfer}
\footnotesize  \setlength{\tabcolsep}{8.0pt}
\centering
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l|c|cccc|ccc|cccccccc} 
\specialrule{.12em}{.1em}{.1em}
\multirow{2}{*}{Method} & \multirow{3}{*}{Type} & \multicolumn{4}{c|}{\uline{ADE}} & \multicolumn{3}{c|}{\uline{Cityscapes}} & \multicolumn{4}{c}{\uline{COCO}} \\
 &  & \multirow{2}{*}{PQ} & \multirow{2}{*}{mask AP} & \multirow{2}{*}{box AP} & \multirow{2}{*}{mIoU} & \multirow{2}{*}{PQ} & \multirow{2}{*}{mask AP} & \multirow{2}{*}{mIoU} &  \multicolumn{2}{c}{PQ} &  \multicolumn{2}{c}{mask AP} &  \multicolumn{2}{c}{box AP} & \multicolumn{2}{c}{mIoU} \\
 &&&&&&&&&&\\
\hline
Mask2Former (T)~\cite{cheng2022masked} & \multirow{7}{*}{Segmentation} & 39.7 & 26.4 & 28.8 & 47.7 & 63.9 & 39.1 & 80.5 & 53.2 & 43.3 & 46.1 & 63.2 \\
Mask2Former (B)~\cite{cheng2022masked} &  & $-$ & $-$ & $-$ & 53.9 & 66.1 & 42.8 & 82.7 & 56.4 & 46.3 & 49.5 & 67.1 \\
Mask2Former (L)~\cite{cheng2022masked} &  & 48.1 & 34.2 & 36.4 & 56.1 & 66.6 & 43.6 & 82.9 & 57.8 & {48.6} & 52.1 & 67.4 \\
OneFormer (L)~\cite{jain2022oneformer} &  & 48.6 & 35.9 & $-$ & 57.0 & 67.2 & 45.6 & ~83.0 & 57.9 & {48.9} & $-$ & 67.4 \\
MaskDINO (L)~\cite{li2022mask} &  & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & 58.3 & {50.6} & 56.2 & 67.5 \\
Pano/SegFormer (B)~\cite{xie2021segformer} &  & $-$ & $-$ & $-$ & 51.0 & $-$ & $-$ & $-$ & 55.4 & $-$ & $-$ & $-$ \\
kMaX-DeepLab (L)~\cite{yu2022k} &  & 48.7 & $-$ & $-$ & 54.8 & $-$ & $-$ & $-$ & {58.1} & $-$ & $-$ & $-$ \\ 
\hline
UViM (L)~\cite{kolesnikov2022uvim} & \multirow{10}{*}{General Purpose} & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & 45.8 & $-$ & $-$ & $-$ \\
Pix2Seq v2 (B)~ &  & $-$$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & 38.2 & $-$ & $-$ \\
GLIPv2 (T)~ &  & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-\lvert$42.0$^\star$ & $-$ & $-$ \\
GLIPv2 (B)~ &  & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-\lvert$45.8$^\star$ & $-$ & $-$ \\
GLIPv2 (H)~ &  & $-$ & $-$ &$-$& $-$ & $-$ & $-$ & & $-$ & $-\lvert$48.9$^\star$ & $-$ & $-$ \\
X-Decoder (T) &  & 41.6 & 27.7 & 28.8 & 51.0 & 61.3 & 36.2& 78.7 & 51.4$\lvert$52.6 & 40.5$\lvert$41.3 & 43.6 & 62.8$\lvert$62.4 \\
{\cellcolor[rgb]{0.961,0.961,0.961}}\ourmodel{} (T) &  & {\cellcolor[rgb]{0.961,0.961,0.961}}\textbf{\textbf{47.2}} & {\cellcolor[rgb]{0.961,0.961,0.961}}\textbf{\textbf{35.1}} & {\cellcolor[rgb]{0.961,0.961,0.961}}\textbf{\textbf{39.4}} & {\cellcolor[rgb]{0.961,0.961,0.961}}\textbf{\textbf{52.2}} & {\cellcolor[rgb]{0.961,0.961,0.961}}\textbf{63.9} & {\cellcolor[rgb]{0.961,0.961,0.961}}\textbf{38.2}  & {\cellcolor[rgb]{0.961,0.961,0.961}}\textbf{80.3} & {\cellcolor[rgb]{0.961,0.961,0.961}}\textbf{55.4}$\lvert -$ & {\cellcolor[rgb]{0.961,0.961,0.961}}\textbf{47.6}$\lvert -$ & {\cellcolor[rgb]{0.961,0.961,0.961}}\textbf{52.0}$\lvert -$ & {\cellcolor[rgb]{0.961,0.961,0.961}}\textbf{64.0}$\lvert -$ \\
% X-Decoder (B) &  & 46.8 & 33.5 & $-$ & 54.6 & $-$ & $-$ & $-$ & $-\lvert$56.2 & $-\lvert$45.8 & $-$ & $-\lvert$66.0 \\
X-Decoder (L) &  & 49.6 & 35.8 & $-$ & 58.1 & $-$ & $-$ & $-$ & $-\lvert$56.9 & $-\lvert$46.7 & $-$ & $-\lvert$67.5 \\


{\cellcolor[rgb]{0.961,0.961,0.961}}\ourmodel{} (L) &  & {\cellcolor[rgb]{0.961,0.961,0.961}}\textbf{53.1~(53.7)} & {\cellcolor[rgb]{0.961,0.961,0.961}}\textbf{42.0~(42.6)} & {\cellcolor[rgb]{0.961,0.961,0.961}}\textbf{46.4~(46.9)} & {\cellcolor[rgb]{0.961,0.961,0.961}}\textbf{58.6~(58.4)} & {\cellcolor[rgb]{0.961,0.961,0.961}\textbf{68.9}}& {\cellcolor[rgb]{0.961,0.961,0.961}\textbf{48.5}}& {\cellcolor[rgb]{0.961,0.961,0.961}\textbf{84.5}}& {\cellcolor[rgb]{0.961,0.961,0.961}\textbf{59.5}}$\lvert -$  & {\cellcolor[rgb]{0.961,0.961,0.961}\textbf{53.2}}$\lvert -$ & {\cellcolor[rgb]{0.961,0.961,0.961}\textbf{58.2}}$\lvert -$ & {\cellcolor[rgb]{0.961,0.961,0.961}\textbf{68.6}} $\lvert -$\\
\specialrule{.12em}{.1em}{.1em}
\end{tabular}
}
\end{table*}


